Special cubulation of strict hyperbolization

We prove that the Gromov hyperbolic groups obtained by the strict hyperbolization procedure of Charney and Davis are virtually compact special, hence linear and residually finite. Our strategy consists in constructing an action of a hyperbolized group on a certain dual CAT(0) cubical complex. As a result, all the common applications of strict hyperbolization are shown to provide manifolds with virtually compact special fundamental group. In particular, we obtain examples of closed negatively curved Riemannian manifolds whose fundamental groups are linear and virtually algebraically fiber.

==> pictures/README.tex <==
Create pictures with Inkscape, with math that looks like the rest of the paper.

For the labels and text, create a text box and input text with dollars as you would do in a normal LaTeX document, typing in Latex.

Copy paste your image in a new file, resize page to selection, save as pdf.
Choose PDF+LaTeX: omit text in pdf and create latex file.

You get a .pdf and a .pdf_tex.

Open the second, and at the bottom locate where they include the .pdf. Make sure to give the right path, based on how things will be organized on overleaf (likely, "pictures/FILENAME.pdf").
OOOOOOR
 For example, if one’s images are in sub-directory images,
add the following to the preamble:
\graphicspath{{pictures/}}



Upload both to Overleaf.

These might be needed in the preamble
\usepackage{graphicx}
\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.5} 
\usepackage{transparent}
\usepackage[adobe-utopia]{mathdesign}


To include the picture
\begin{figure}[h]
\centering
\def\svgwidth{\columnwidth}
\input{pictures/FILENAME.pdf_tex}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

To scale better
\usepackage{calc}...
\begin{figure}
\centering
\def\svgscale{1.5}
\input{image.pdf_tex}
\caption{Caption}
\label{fig:my_label}
\end{figure}

REFERENCES
https://ctan.mirrors.hoobly.com/info/svg-inkscape/InkscapePDFLaTeX.pdf

https://wiki.inkscape.org/wiki/LaTeX#:~:text=Recent%20versions%20of%20Inkscape%20(since,%3ERender%2D%3ELaTeX%20Formula.&text=Alternatively%2C%20you%20can%20use%20the,slightly%20more%20polished%20input%20interface

https://ctan.org/tex-archive/info/svg-inkscape


